Accelerating Dedispersion using Many-Core Architectures

Astrophysical radio signals are excellent probes of extreme physical processes that emit them. However, to reach Earth, electromagnetic radiation passes through the ionised interstellar medium (ISM), introducing a frequency-dependent time delay (dispersion) to the emitted signal. Removing dispersion enables searches for transient signals like Fast Radio Bursts (FRB) or repeating signals from isolated pulsars or those in orbit around other compact objects. The sheer volume and high resolution of data that next generation radio telescopes will produce require High-Performance Computing (HPC) solutions and algorithms to be used in time-domain data processing pipelines to extract scientifically valuable results in real-time. This paper presents a state-of-the-art implementation of brute force incoherent dedispersion on NVIDIA GPUs, and on Intel and AMD CPUs. We show that our implementation is 4x faster (8-bit 8192 channels input) than other available solutions and demonstrate, using 11 existing telescopes, that our implementation is at least 20 faster than real-time. This work is part of the AstroAccelerate package.

==> table-cpu-hardware.tex <==
\begin{table}[htb!]
	\caption{Hardware specifications.}
	\begin{center}
	%\centering
	\begin{tabular}{|l|r|r|}
	\hline
	\textbf{} & \textbf{Xeon Gold 6140} & \textbf{Xeon Phi 7290}\\
	\hline
	\# of Cores & 18 & 72 \\
	Base clock Frequency & 2.1 GHz & 1.5 GHz\\
	Cache size & 24.75 MB L3 & 36 MB L2\\
	\hline
	\end{tabular}
	\label{tab:hardware} 
	\end{center}
\end{table}

==> table-results.tex <==
\begin{table}[htb!]
\centering
\caption{\label{tab:results}Time results (in seconds) of the plans for different channels and code implementations.}
\begin{tabular}{llrrrr}
\toprule
Code     & CPU/GPU       & 512   & 1024  & 2048  & 4096  \\
\midrule
\multirow{2}{*}{Sclocco} & Titan XP      & 0.126 & 0.248 & 0.438 & 0.820 \\
						 & Titan V		 & 0.077 & 0.137 & 0.205 & 0.360\\
\midrule
\multirow{2}{*}{Barsdell}& Titan XP      & 0.179 & 0.345 & 0.632 & 1.187 \\
                         & Titan V       & 0.152 & 0.296 & 0.568 & 1.115 \\
\midrule
Our & Xeon-Phi 7290 & 0.222 & 0.354 & 0.616 & 1.145 \\
\bottomrule
\end{tabular}
\end{table}
